We are More than Our Joints: Predicting how 3D Bodies Move

A key step towards understanding human behavior is the prediction of 3D human motion. Successful solutions have many applications in human tracking, HCI, and graphics. Most previous work focuses on predicting a time series of future 3D joint locations given a sequence 3D joints from the past. This Euclidean formulation generally works better than predicting pose in terms of joint rotations. Body joint locations, however, do not fully constrain 3D human pose, leaving degrees of freedom undefined, making it hard to animate a realistic human from only the joints. Note that the 3D joints can be viewed as a sparse point cloud. Thus the problem of human motion prediction can be seen as point cloud prediction. With this observation, we instead predict a sparse set of locations on the body surface that correspond to motion capture markers. Given such markers, we fit a parametric body model to recover the 3D shape and pose of the person. These sparse surface markers also carry detailed information about human movement that is not present in the joints, increasing the naturalness of the predicted motions. Using the AMASS dataset, we train MOJO, which is a novel variational autoencoder that generates motions from latent frequencies. MOJO preserves the full temporal resolution of the input motion, and sampling from the latent frequencies explicitly introduces high-frequency components into the generated motion. We note that motion prediction methods accumulate errors over time, resulting in joints or markers that diverge from true human bodies. To address this, we fit SMPL-X to the predictions at each time step, projecting the solution back onto the space of valid bodies. These valid markers are then propagated in time. Experiments show that our method produces state-of-the-art results and realistic 3D body animations. The code for research purposes is at https://yz-cnsdqz.github.io/MOJO/MOJO.html

==> sec4-experiment-v-1.tex <==
\section{Experiment}
\label{sec:experiments}


\subsection{Datasets}
For training, we use the {\bf AMASS}~\cite{AMASS:ICCV:2019} dataset. 
Specifically, we train the models on {\bf CMU}~\cite{mocap_cmu} and {\bf MPI HDM05}~\cite{muller2007documentation}, and test models on {\bf ACCAD}~\cite{accad} and {\bf BMLhandball}~\cite{helm2017motion,helm2020integrating}. 
%The {\bf CMU} dataset contains 551.56 minutes of motion from 106 subjects, and the {\bf MPI HDM05} dataset contains 144.54 minutes of motion from 4 subjects. The {\bf ACCAD} dataset contains 26.74 minutes of motions from 20 subjects, including walking, running, kicking, and other coarse-grained actions. The {\bf BMLhandball} dataset contains 101.98 minutes of hand ball playing from 10 subjects, in which most motions are fine-grained such as waving and picking up objects.
%
This gives 696.1 minutes of training motion from 110 subjects and
128.72 minutes of test motion from 30 subjects.
The test sequences include a wide range of actions. 
%
To unify the sequence length and world coordinates, we canonicalize {\bf AMASS} as follows: \textit{First}, we trim the original sequences into 480-frame (4-second) subsequences, and downsample them from 120fps to 15fps. The condition sequence ${\bm X}$ contains 15 frames (1s) and the future sequence $\bm Y$ contains 45 frames (3s). \textit{Second}, we unify the world coordinates as in \cite{zhang2020perpetual}. For each subsequence, we reset the world coordinate to the SMPL-X~\cite{SMPL-X:2019} body mesh in the first frame: The horizontal X-axis points in the direction from the left hip to the right hip, the Z-axis is the negative direction of gravity, and the Y-axis is pointing forward. The origin is set to to the body's global translation.


To compare our method with SOTA stochastic motion prediction methods, we additionally perform skeleton-based motion prediction on the {\bf Human3.6M} dataset~\cite{h36m_pami} and the {\bf HumanEva-I} dataset~\cite{sigal2010humaneva}, following the experimental setting of Yuan et al.~\cite{yuan2020dlow}.
% On {\bf Human3.6M} we use the 17-joint skeleton, perform training on subjects (S1, S5, S6, S7, S8), and perform testing on (S9 and S11). The condition sequence ${\bm X}$ has 25 frames (0.5s), and the predicted sequence ${\bm Y}$ has 100 frames (2s).
% On {\bf HumanEva-I} we use a 15-joint skeleton. 
% The condition sequence ${\bm X}$ has 15 frames (0.25s), and the predicted sequence ${\bm Y}$ has 60 frames (1s).


\subsection{Baselines}
For fair comparison on {\bf Human3.6M} and {\bf HumanEva-I}, we use the same setting of the CVAE as in DLow~\cite{yuan2020dlow}, except that we add our latent DCT space into the model and train it with the robust KLD term. For sampling, we apply a set of DLow models $\{\textbf{Q}_w\}$ on the lowest $L$ bands, as in Sec.~\ref{sec:generative_model}. We denote this modified model as `VAE+DCT+$L$', which is used to verify the effectiveness of the latent DCT space. Absence of the suffix `+$L$' indicates sampling from $\mathcal{N}(0, {\bm I})$ at all frequency bands.

Unlike the baseline, MOJO predicts surface markers. 
%Without explicitly mentioning, 
Unless mentioned, we use the CMU layout with 41 markers.
MOJO has several components.
`MOJO-DCT' is the model without DCT, but with the same latent space as the CVAE in DLow. 
`MOJO-proj' is the model without  recursive projection.
Note that the suffixes can be concatenated; e.g.~`MOJO-DCT-proj' is the model without the latent DCT space and without the recursive projection scheme.
% Moreover, we use `MOJO w. J.' to denote a traditional pipeline, which first predicts joints and then fits the body mesh to the predicted joints. Its generative model architecture is identical to MOJO.



\subsection{Evaluation of Stochastic Motion Prediction}
\label{sec:stochastic_prediction}
\subsubsection{Metrics}

\myparagraph{Diversity.} 
We use the same diversity measure as \cite{yuan2020dlow}, which is the average pair-wise distance between all generated sequences. 

\myparagraph{Prediction accuracy.} 
As in~\cite{yuan2020dlow}, we use the average distance error (\textit{ADE}) and the final distance error (\textit{FDE}) to measure the minimum distance between the generated motion and the ground truth, w.r.t. frame-wise difference and the final frame difference, respectively
Additionally, we  use \textit{MMADE} and \textit{MMFED} to evaluate  prediction accuracy when the input sequence slightly changes;  see  Appendix.

\myparagraph{Motion Frequency.} Similar to \cite{hernandez2019human}, we compute the frequency spectra entropy (\textit{FSE}) to measure motion frequency in the Fourier domain, which is given by the averaged spectra entropy minus the ground truth. 
A higher value indicates the generated motions contain more motion detail. 
Note that high frequency can also indicate noise, and hence this metric is jointly considered with the prediction accuracy.



\subsubsection{Results}
In the following experiments, we generate 50 different future sequences based on each input sequence, as in~\cite{yuan2020dlow}. 

\myparagraph{Skeleton-based motion prediction.}
The results are shown in Tab.~\ref{tab:skeleton_compare}. 
Our latent DCT space improves on the state-of-the-art. Specifically, the diversity is improved by a large margin, while the prediction accuracy are comparable to the baseline.
The performance w.r.t.~MMADE and MMFDE is slightly inferior. 
A probable reason is VAE+DCT uses high-frequency components to generate motions, which makes motion prediction sensitive to slight changes of the input.
\textcolor{red}{
Another probable reason is the mismatched similarity measure. 
In MMADE and MMFDE, similar motions are selected according to the L2 distance of the last frame. However, motions in VAE+DCT are represented by latent frequencies, and better to be compared w.r.t. frequencies. }
%\yan{I am not sure whether this "another probable reason..." is necessary.}
Additionally, direct sampling from the standard normal distribution does not exploit the advantage of the latent DCT space effectively, since the information at low-frequency bands is ignored.
Moreover, the diversity increases sublinearly as DLow is applied on more low-frequency bands, which indicates a lower-frequency band carries more information than a higher-frequency band. This fits the energy compaction property of DCT.


\begin{table*}[t!]
    \scriptsize
    \centering
    \begin{tabular}{lrccccrcccc}
        \toprule
        &\multicolumn{5}{c}{\textbf{Human3.6M}~\cite{h36m_pami}} & \multicolumn{5}{c}{\textbf{HumanEva-I}~\cite{sigal2010humaneva}}\\
        \cmidrule(lr){2-6} \cmidrule(lr){7-11}
        Method & \textit{Diversity}$\uparrow$ & \textit{ADE}$\downarrow$ & \textit{FDE}$\downarrow$ & \textit{MMADE}$\downarrow$ & \textit{MMFDE}$\downarrow$ & \textit{Diversity}$\uparrow$ & \textit{ADE}$\downarrow$ & \textit{FDE}$\downarrow$ & \textit{MMADE}$\downarrow$ & \textit{MMFDE}$\downarrow$ \\
        \midrule
        Pose-Knows~\cite{walker2017pose} & 6.723 & 0.461 & 0.560 & 0.522 & 0.569 & 2.308 & 0.269 & 0.296 & 0.384 & 0.375\\
        MT-VAE~\cite{yan2018mt} & 0.403 & 0.457 & 0.595 & 0.716 & 0.883 & 0.021 & 0.345 & 0.403 & 0.518 & 0.577\\
        HP-GAN~\cite{barsoum2018hp} & 7.214 & 0.858 & 0.867 & 0.847 & 0.858 & 1.139 & 0.772 & 0.749 & 0.776 & 0.769 \\
        Best-of-Many~\cite{bhattacharyya2018accurate} & 6.265 & 0.448 & 0.533 & 0.514 & 0.544 & 2.846 & 0.271 & 0.279 & 0.373 & 0.351\\
        GMVAE~\cite{dilokthanakul2016deep} & 6.769 & 0.461 & 0.555 & 0.524 & 0.566 & 2.443 & 0.305 & 0.345 & 0.408 & 0.410\\
        DeLiGAN~\cite{gurumurthy2017deligan} & 6.509 & 0.483 & 0.534 & 0.520 & 0.545 & 2.177 & 0.306 & 0.322 & 0.385 & 0.371\\
        DSF~\cite{yuan2019diverse} & 9.330 & 0.493 & 0.592 & 0.550 & 0.599 & 4.538 & 0.273 & 0.290 & 0.364 & 0.340\\
        DLow~\cite{yuan2020dlow} & 11.730 & 0.425 & 0.518 & \textbf{0.495} & \textbf{0.532} & 4.849 & 0.246 & 0.265 & \textbf{0.360} & \textbf{0.340} \\
        \midrule
        VAE+DCT & 3.462 & 0.429 & 0.545 & 0.525 & 0.581 & 0.966 & 0.249 & 0.296 & 0.412 & 0.445 \\
        VAE+DCT+5 & 12.579 & \textbf{0.412} & \textbf{0.514} & 0.497 & 0.538 & 4.181 & \textbf{0.234} & \textbf{0.244} & 0.369 & 0.347 \\
        VAE+DCT+20 & \textbf{15.920} & 0.416 & 0.522 & 0.502 & 0.546 & \textbf{6.266} & 0.239 & 0.253 & 0.371 & 0.345 \\
        \bottomrule
    \end{tabular}
    \vspace{-0.1in}
    \caption{Comparison between our method and state-of-the-art. The symbol $\downarrow$ (or $\uparrow$) denotes whether results that are higher (or lower) the better, respectively. Best results are in boldface.  }
 %   \vspace{-1mm}
    \label{tab:skeleton_compare}
\end{table*}

We repeat this experiment, replacing the joints with markers.
This is not the full MOJO method because we do not use the re-projection scheme.
Again, we find the DCT formulating improves diversity and accuracy. 
See Appendix for details.



\subsection{Evaluation of Motion Realism}

\subsubsection{Metrics}

\textcolor{red}{motivate this section. why new metrics? discuss limits of the ohter metrics.}

\myparagraph{Rigid body deformation.}
\textcolor{red}{I have no idea what this is experiment is about or what any of this has to do with deformation or what sort of deformation is being measured and why.}
We measure the markers on the head, the upper torso and the lower torso, respectively.
Specifically, according to {\bf CMU}~\cite{mocap_cmu}, we measure (`LFHD', `RFHD', `RBHD', `LBHD') for the head, (`RSHO', `LSHO', `CLAV', `C7') for the upper torso, and (`RFWT', `LFWT', `LBWT', `RBWT') for the lower torso.
% The deformation is evaluated by the variations of pairwise L2 distances of markers. 
For each rigid body part $P$, the deformation score is the variations of marker pair-wise distances, and is calculated by
\begin{equation}
    s_d(P) = \mathbb{E}_{\bm Y}\left[ \sum_{(i,j)\in P} \sigma_t(|{\bm v}^t_i-{\bm v}_j^t|^2) \right],
    \label{eq:deformation}
\end{equation}
in which ${\bm v}^t_i$ denotes the location of the marker $i$ at time $t$, $\sigma_t$ denotes the standard deviation along the time dimension, and $\mathbb{E}_{\bm Y}[\cdot]$ denotes averaging the scores of different predicted sequences.


\myparagraph{Foot skating ratio.}
Foot skating is measured based on the two markers on the feet calcaneus (`LHEE' and `RHEE' in \textbf{CMU}~\cite{mocap_cmu}). 
We consider foot skating to have occurred, when both foot markers are close enough to the ground (within 5cm) and simultaneously exceed a speed limit (5mm between two consecutive frames or 75mm/s).
We report the averaged ratio of frames with foot skating.


\myparagraph{Perceptual score.}
We render the generated body meshes as well as the ground truth, and perform a perceptual study on Amazon Mechanical Turk.
Subjects see a motion sequence and the statement ``The human motion is natural and realistic."  They evaluate this on a six-point Likert scale from `strongly disagree` (1) to `strongly agree' (6). 
Each individual video is rated by three subjects.
We report mean values and standard deviations for each method and each dataset.


\subsubsection{Results}

In the following, we randomly choose 60 different sequences from {\bf ACCAD} and {\bf BMLhandball}, respectively. Based on each sequence, we generate 15 future sequences.
Figure \ref{fig:bm_diverse} shows some generated 3D body motions. 
The motions generated by MOJO contain finer-grained body movements.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/bm-vis-1.pdf}
        \vspace{-0.25in}
    \caption{Visualization of 3D body motions. Bodies in gray-green and red denote the input and the generated motion, respectively. The solid and dash image borders denote the results from MOJO-DCT and MOJO, respectively.}       %\vspace{-5mm}
    \label{fig:bm_diverse}
\end{figure}


\begin{table}
    \scriptsize
    \centering
    \begin{tabular}{lcccccc}
        \toprule
          & \multicolumn{3}{c}{\textbf{ACCAD}~\cite{accad}} & \multicolumn{3}{c}{\textbf{BMLHandball}~\cite{helm2017motion,helm2020integrating}}\\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7}
        Method & Head & Up.~T. & Low.~T. & Head & Up.~T. & Low.~T.\\
        \midrule
        MOJO-DCT-proj & 76.3 & 102.2 & 99.4 & 86.0 & 105.3 & 83.3\\
        MOJO-proj & \textbf{70.3} & \textbf{80.7} & \textbf{76.7} & \textbf{68.3} & \textbf{77.7} & \textbf{63.2} \\
        \midrule
        MOJO-DCT & 1.32 & 34.0 & 6.97 & \textbf{1.32} & \textbf{43.1} & \textbf{6.97}\\
        MOJO & \textbf{1.30} & \textbf{32.7} & \textbf{6.76} & 1.40 & 44.3 & 7.64\\
        \bottomrule
    \end{tabular}
    \vspace{-0.1in}
   \caption{Evaluation on rigid part deformation in motion (head, Upper Torso, Lower Torso). All scores are in the scale of $10^{-3}$; lower is better. Best results are in boldface. }
  %  \vspace{-1mm}
    \label{tab:deformation}
\end{table}



\begin{table}
    \scriptsize
    \centering
    \begin{tabular}{lcccc}
        \toprule
          & \multicolumn{2}{c}{\textbf{ACCAD}~\cite{accad}} & \multicolumn{2}{c}{\textbf{BMLHandball}~\cite{helm2017motion,helm2020integrating}}\\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5}
        Method & foot skate & percep.~score & foot skate & percep.~score\\
        \midrule
        MOJO-DCT & 0.341 & \textbf{4.15}$\pm$1.38 & 0.077 & 4.00$\pm$1.26\\
        MOJO & \textbf{0.278} & 4.07$\pm$\textbf{1.31} & \textbf{0.066} & \textbf{4.17}$\pm$\textbf{1.23}\\
        \midrule
        ground truth&  \textit{0.067} & \textit{4.82}$\pm$\textit{1.08} & \textit{0.002} & \textit{4.83}$\pm$\textit{1.05}\\
        \bottomrule
    \end{tabular}
    \vspace{-0.1in}
    \caption{\textcolor{red}{Evaluation on rigid part deformation in motion. All scores are in the scale of $10^{-3}$, and the lower the better. Best results are in boldface. }}
    %\vspace{-1mm}
    \label{tab:skating_userstudy}
\end{table}





% \begin{table}
%     \scriptsize
%     \centering
%     \begin{tabular}{lcc}
%         \toprule
%         Method &{\textbf{ACCAD}~\cite{accad}} & {\textbf{BMLHandball}~\cite{helm2017motion,helm2020integrating} }\\
%         \midrule
%         MOJO-DCT & 0.341 & 0.077\\
%         MOJO & \textbf{0.278} & \textbf{0.066}\\
%         \midrule
%         ground truth & \textit{0.067} & \textit{0.002}\\
%         \bottomrule
%     \end{tabular}
%     \caption{Comparison between methods w.r.t. foot skating. Best results are in boldface. }
%     \vspace{-1mm}
%     \label{tab:skating}
% \end{table}

% \begin{table}
%     \scriptsize
%     \centering
%     \begin{tabular}{lcc}
%         \toprule
%         Method &{\textbf{ACCAD}~\cite{accad}} & {\textbf{BMLHandball}~\cite{helm2017motion,helm2020integrating}}\\
%         \midrule
%         MOJO-DCT & \textbf{4.15}$\pm$1.38 & 4.00$\pm$1.26\\
%         MOJO & 4.07$\pm$\textbf{1.31} & \textbf{4.17}$\pm$\textbf{1.23}\\
%         \midrule
%         ground truth & \textit{4.82}$\pm$\textit{1.08} & \textit{4.83}$\pm$\textit{1.05}\\
%         \bottomrule
%     \end{tabular}
%     \caption{Perceptual scores from the user study. Best results of each model are in boldface. Note that the score ranges from 1 to 6. }        \vspace{-4mm}
%     \label{tab:userstudy}
% \end{table}




% \begin{table*}[t!]
%     \footnotesize
%     \centering
%     \begin{tabular}{lllllllllllll}
%         \toprule
%         &\multicolumn{6}{c}{\textbf{ACCAD}~\cite{accad}} & \multicolumn{6}{c}{\textbf{BMLHandball}~\cite{helm2017motion,helm2020integrating}}\\
%         \cmidrule(lr){2-7} \cmidrule(lr){8-13}
%         Method & \textit{Diversity}$\uparrow$ & \textit{ADE}$\downarrow$ & \textit{FDE}$\downarrow$ & \textit{MMADE}$\downarrow$ & \textit{MMFDE}$\downarrow$ & \textit{BDF}$\downarrow$ & \textit{Diversity}$\uparrow$ & \textit{ADE}$\downarrow$ & \textit{FDE}$\downarrow$ & \textit{MMADE}$\downarrow$ & \textit{MMFDE}$\downarrow$ & \textit{BDF}$\downarrow$ \\
%         \midrule
%         MOJO w. J. & \textbf{21.363} & \textbf{1.184} & 2.010 & \textbf{1.291} & \textbf{2.067} & 0.185 & \textbf{19.091} & \textbf{0.930} & \textbf{1.132} & \textbf{1.000} & \textbf{1.156} & 0.205\\
%         MOJO & 20.676 & {1.214} & \textbf{1.919} & 1.306 & 2.080 & \textbf{0} & 16.806 & {0.949} & {1.139} & {1.001} & {1.172} & \textbf{0}\\
%         \bottomrule
%     \end{tabular}
%     \caption{Comparison between marker-based and joint-based representations. Evaluations are based on the joint locations. {\em BDF} denotes the bone deformation w.r.t. meters. The best results are in boldface. }        
%     \vspace{-3mm}
%     \label{tab:jts_vs_marker}
% \end{table*}




\begin{table*}[t!]
    \scriptsize
    \centering
    \begin{tabular}{lllllllllllll}
        \toprule
        &\multicolumn{6}{c}{\textbf{ACCAD}~\cite{accad}} & \multicolumn{6}{c}{\textbf{BMLHandball}~\cite{helm2017motion,helm2020integrating}}\\
        \cmidrule(lr){2-7} \cmidrule(lr){8-13}
        Method & \textit{Diversity}$\uparrow$ & \textit{ADE}$\downarrow$ & \textit{FDE}$\downarrow$ & \textit{MMADE}$\downarrow$ & \textit{MMFDE}$\downarrow$ & \textit{BDF}$\downarrow$ & \textit{Diversity}$\uparrow$ & \textit{ADE}$\downarrow$ & \textit{FDE}$\downarrow$ & \textit{MMADE}$\downarrow$ & \textit{MMFDE}$\downarrow$ & \textit{BDF}$\downarrow$ \\
        \midrule
        joints w/o proj. & {21.363} & {1.184} & 2.010 & {1.291} & {2.067} & 0.185 & \textbf{19.091} & {0.930} & {1.132} & {1.000} & {1.156} & 0.205\\
        joints  & 21.106 & 1.192 & 2.022 & 1.299 & 2.076 & 0 & 18.954 & 0.934 & 1.138 & 1.003 & 1.157 & 0 \\
        CMU 41 & 20.676 & {1.214} & {1.919} & 1.306 & 2.080 & {0} & 16.806 & {0.949} & {1.139} & {1.001} & {1.172} & {0}\\
        SSM2 67 & \textbf{24.373} & \textbf{1.124} & \textbf{1.699} & \textbf{1.227} & \textbf{1.838} & 0 & 18.778 & \textbf{0.924} & \textbf{1.099} & \textbf{0.975} & \textbf{1.149} & 0\\
        joints + CMU 41 & 20.988 & 1.187 & 1.841 & 1.308 & 1.967 & 0 & 13.982 & 0.943 & 1.190 & 0.990 & 1.194 & 0\\
        joints + SSM2 67 & 23.504 & 1.166 & 1.892 & 1.276 & 1.953 & 0 & 16.483 & 0.950 & 1.146 & 0.999 & 1.189 & 0\\
        \bottomrule
    \end{tabular}
    \vspace{-0.1in}
    \caption{Comparison between marker-based and joint-based representations. Evaluations are based on the joint locations. {\em BDF} denotes the bone deformation w.r.t. meters. The best results are in boldface. }        
    %\vspace{-3mm}
    \label{tab:comparison_jts_markers}
\end{table*}


\myparagraph{Rigid body deformation.}
The results are shown in Tab. \ref{tab:deformation}.
With the standard RNN inference, the consistent superiority of `MOJO-proj` to `MOJO-DCT-proj` can indicate that the latent DCT space captures interactions between markers more effectively.
With the recursive projection scheme, we can see the body shape is preserved.
This verifies the effectiveness of the projection scheme, which constrains the motion prediction process within a valid body space.


\myparagraph{Foot skating and perceptual score.}
The results are presented in Tab. \ref{tab:skating_userstudy}.
The model with DCT produces fewer foot skating artifacts. 
A probable reason is that high-frequency components in the DCT space can better model the foot movements.
W.r.t. user study, MOJO performs slightly worse than MOJO-DCT on {\bf ACCAD}, but outperforms it significantly on {\bf BMLhandball}. 
A probable reason is that most actions in {\bf ACCAD} are coarse-grained, whereas most actions in {\bf BMLhandball} are fine-grained. 
The advantage of modelling finer-grained motion of the DCT latent space is more easily perceived in {\bf BMLhandball}.




\subsection{Comparison between Body Representations}
The body in motion can be represented by locations of joints, markers with different placements, and their combinations. Here we perform a systematic comparison between them.
For the joint-based representation, we use the SMPL~\cite{SMPL:2015} joint locations from {\bf CMU} and {\bf MPI HDM05} to train a CVAE as in MOJO.
A traditional pipeline is to first predict all joints in the future, and then fit the body mesh. Here we also test the performance when applying the recursive body re-projection scheme based on joints.
For fair quantitative evaluation, the metrics are calculated based on the joints of the fitted body meshes.
We re-calculate the diversity and prediction accuracy metrics w.r.t.~the joint locations. 
Also, we measure the bone deformation (BDF) of the eight  limb bones, according to Eq.~\eqref{eq:deformation} working on joints.


We randomly choose 60 sequences from each test set and generate 50 future motions based on each sequence. 
Results are presented in Tab.~\ref{tab:comparison_jts_markers}.
The first two rows show that the motion naturalness is improved by the recursive projection, which eliminates the bone deformation. Although the result without projection is slightly better on other measures, the projection scheme completely removes bone deformation and does not produce false poses as in Fig.~\ref{fig:fit_jts}. 
Additionally, using more markers (SSM2 placement with 67 markers) significantly improves performance across the board. 
This shows that the marker distribution is important for motion prediction and that more markers is better.
While MOJO works with markers, joints, or combination of both, the combination of joints and markers does not produce better performance. 
%A denser marker placement gives better performance. 
Note that the joints are never directly observed, but rather are inferred from the markers by commercial mocap systems. Hence, we argue that the joints do not add independent information. 


Figure \ref{fig:fit_jts} shows the risk of the traditional joint-based pipeline. At the last predicted frame, the character cannot be fit to the joints  due to unrealistic bone lengths (notice the right calf bone).

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/body_deform.png}
    \vspace{-0.25in}
    \caption{Fitting a character to predicted joints. From left to right: The first predicted frame, the middle frame, and the last frame.}
    \label{fig:fit_jts}
\end{figure}










% \subsection{Markers vs Joints}

% To investigate the benefits of our MOJO solution, here we compare it with its counterpart traditional pipeline MOJO w. J., which is trained with the SMPL~\cite{SMPL:2015} joint locations from {\bf CMU} and {\bf MPI HDM05}. Thereafter, the ground truth body mesh is fitted to the predicted joints.

% For performance evaluation, we re-calculate the diversity and prediction accuracy metrics w.r.t.~the joint locations. 
% Also, we measure the bone deformation (BDF) of the eight  limb bones, according to Eq.~\eqref{eq:deformation} working on joints.
% For the results from MOJO, we retrieve the corresponding SMPL joints from the SMPL-X body mesh for fair comparison.


% We randomly choose 60 sequences from each test set and generate 50 future motions based on each sequence. 
% Results are presented in Tab.~\ref{tab:jts_vs_marker}.
% We can see their performance is  comparable. However, MOJO w. J. can lead to bone deformation, making it fail to fit a character to the joints.
% Figure \ref{fig:fit_jts} shows such an example. At the last predicted frame, the character cannot be fitted in due to unrealistic bone lengths (notice the right calf bone).


% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/body_deform.png}
%     \caption{Fitting a character to predicted joints. From left to right: The first predicted frame, the middle frame, and the last frame.}
%     \vspace{-3mm}
%     \label{fig:fit_jts}
% \end{figure}












